Phase-Bounded Broadcast Networks over Topologies of Communication

We study networks of processes that all execute the same finite state protocol and that communicate through broadcasts. The processes are organized in a graph (a topology) and only the neighbors of a process in this graph can receive its broadcasts. The coverability problem asks, given a protocol and a state of the protocol, whether there is a topology for the processes such that one of them (at least) reaches the given state. This problem is undecidable. We study here an under-approximation of the problem where processes alternate a bounded number of times $k$ between phases of broadcasting and phases of receiving messages. We show that, if the problem remains undecidable when $k$ is greater than 6, it becomes decidable for $k=2$, and EXPSPACE-complete for $k=1$. Furthermore, we show that if we restrict ourselves to line topologies, the problem is in $P$ for $k=1$ and $k=2$.

==> Figures/local-reordening.tex <==
\tikzset{box/.style={draw, minimum width=4em, text width=4.5em, text centered, minimum height=17em}}

\begin{tikzpicture}[-, >=stealth', shorten >=1pt,node distance=2.5cm,on grid,auto, initial text = {}]
\end{tikzpicture}

==> Figures/prot-undec-simul-M.tex <==
\tikzset{box/.style={draw, minimum width=4em, text width=4.5em, text centered, minimum height=17em}}

\begin{tikzpicture}[-, >=stealth', shorten >=1pt,node distance=2cm,on grid,auto, initial text = {}] 
\end{tikzpicture}

==> for-me.tex <==

%\begin{figure}
%	\begin{minipage}[c]{0.32\linewidth}
%		\resizebox*{1.0\linewidth}{!}{
%		\input{Figures/prot-P1}
%	}
%		\subcaption{$\PP_1$.}
%	\end{minipage}
%	\hfill
%	\begin{minipage}[c]{0.32\linewidth}
%		\resizebox*{1.0\linewidth}{!}{
%			\input{Figures/prot-P1}
%		}
%		\subcaption{$\PP_1$.}
%	\end{minipage}
%	\hfill
%	\begin{minipage}[c]{0.32\linewidth}
%	\resizebox*{1.0\linewidth}{!}{
%		\input{Figures/prot-P1}
%	}
%	\subcaption{$\PP_1$.}
%\end{minipage}
%\end{figure}


\begin{figure}
	\begin{minipage}[c]{0.45\linewidth}
		\resizebox*{0.8\linewidth}{!}{
			\input{Figures/prot-head.tex}
		}
		\subcaption{Protocol for $v_0$.}
	\end{minipage}
\hfill
	\begin{minipage}[c]{0.47\linewidth}
		\resizebox*{1.0\linewidth}{!}{
		\input{Figures/prot-tail.tex}
	}
		\subcaption{Protocol for $v_5$.}
	\end{minipage}
\end{figure} 


\begin{figure}
	\begin{center}
		\input{Figures/lines-example1.tex}
	\end{center}
\caption{If someone else than $v_0$ starts...}
\end{figure} 

%\begin{figure}
%	\begin{minipage}[c]{0.4\linewidth}
%		\begin{center}
%			\resizebox*{!}{0.4\columnwidth}{
%				\input{Figures/lines-example2.tex}
%			}
%		\end{center}
%	\subcaption{Example 1}
%	\end{minipage}
%	\begin{minipage}[c]{0.4\linewidth}
%		\begin{center}
%			\resizebox*{!}{0.4\columnwidth}{
%			\input{Figures/lines-example5.tex}
%			}
%		\subcaption{Example 2}
%		\end{center}
%	\end{minipage}
%	\caption{Examples of wrong transimission}
%\end{figure} 

%\begin{figure}
%	\begin{minipage}[c]{0.4\linewidth}
%		\resizebox*{!}{0.9\columnwidth}{
%		\input{Figures/lines-example3.tex}
%		}
%		\subcaption{Transmission.}
%	\end{minipage}
%	\hfill
%	\begin{minipage}[c]{0.4\linewidth}
%		\hspace{-15mm}
%		\resizebox*{!}{0.9\columnwidth}{
%			\input{Figures/lines-example4.tex}
%		}
%		\subcaption{Transmission.}
%	\end{minipage}
%	\caption{How the transmission happens}
%\end{figure} 


\begin{figure}
	\begin{center}
		\input{Figures/lines-example6.tex}
	\end{center}
	\caption{End of the simulation}
\end{figure} 

==> inP-proofs-old.tex <==
\subsection{Proofs of \cref{subsec:coverLine-inP}}\label{appendix:proof-inP}
%\lugtext{----- à déplacer -----}
%For a 2-phase bounded protocol $\PP= (Q, \Sigma, \qinit, \Delta)$ and we denote $\Delta_{!!}$ [resp. $\Delta_{\tau}$] the set of broadcasts transitions [resp. internal transitions], i.e. $\Delta_{!!} = \Delta\cap(Q\times !! \Sigma \times Q)$ [resp. $\Delta_{\tau} = \Delta \cap (Q\times \set{\tau} \times Q)$].
%\lugtext{-------------------}
\subsubsection{Proof of \cref{lemma:CoverLine-2pb-inP:execution-shape-2}}\label{appendix:subsec:CoverLine-inP:lemma:shape}
Let $q_f \in Q$ be a coverable state.
We fix $\Gamma$ with $\Vert{\Gamma} = \set{v_1, \dots, v_\ell}$ the line topology such that there exists $\rho = C_0 \trans \cdots \trans C_n$ with $C_n = (\Gamma, L_n)$ and $L_n(v_N) = q_f$ for some $v_N \in \Vert{\Gamma}$. We suppose wlog that $N \geq 3$ and $N \leq \ell- 2$, otherwise, we can just add artificial nodes not issuing any transition in the execution.

We start by proving the following lemma.
\begin{lemma}\label{lemma:CoverLine-2pb-inP:execution-shape-1}
There exists $\rho' = C'_0 \trans^\ast C'_n$ such that $C'_n = (\Gamma, L'_n)$ with $L'_n(v_N)= q_f$, and
	\begin{itemize}
		\item for all $1 \leq i \leq N-2$, $\lastBroadcast{v_i}{\rho'} \leq \firstBroadcast{v_{i+1}}{\rho'}$;
		\item for all $N+2 \leq i \leq \ell$, $\lastBroadcast{v_i}{\rho'} \leq \firstBroadcast{v_{i-1}}{\rho'}$.
	\end{itemize} 
\end{lemma}

\paragraph{Proof of \cref{lemma:CoverLine-2pb-inP:execution-shape-1}.}

To prove \ref{lemma:CoverLine-2pb-inP:execution-shape-1}, we give two symmetric lemmas.
\begin{lemma}\label{lemma:CoverLine-2pb-inP:execution-shape-right}
	Let $\rho = C_0\trans^\ast C$ with $C = (\Gamma, L)$ and $1 \leq K < \ell$. 
	There exists $\rho' = C_0  \trans^\ast C'$ such that $C' = (\Gamma, L')$, and 
	\begin{itemize}
	\item for all $v \in \set{v_{K+1}, \dots, v_\ell}$, $L'(v) = L(v)$;
	\item for all $1 \leq i \leq K-1$, $\lastBroadcast{v_i}{\rho'} \leq \firstBroadcast{v_{i+1}}{\rho'}$;
	\item for all $K + 1\leq i \leq \ell$, $\lastBroadcast{v_i}{\rho'} \leq \firstBroadcast{v_{i+1}}{\rho'}$ if and only if $\lastBroadcast{v_i}{\rho} \leq \firstBroadcast{v_{i+1}}{\rho}$.
	\end{itemize}
\end{lemma}
\begin{proof}
	Let $\rho = C_0 \trans^\ast C = (\Gamma, L)$ and $1 \leq K < \ell$. 
%	Denote $1 \leq k \leq K$ the smallest index such that $\lastBroadcast{v_k}{\rho} > \firstBroadcast{v_{k+1}}{\rho}$. We show how to build $\rho_k$ such that:
%	\begin{itemize}
%		\item for all $v \in \set{v_{k+1}, \dots, v_\ell}$, $L'_n(v) = L_n(v)$;
%		\item for all $1 \leq i \leq k-1$, $\lastBroadcast{v_i}{\rho'} \leq \firstBroadcast{v_{i+1}}{\rho'}$;
%		\item for all $k \leq i \leq \ell$, $\lastBroadcast{v_i}{\rho'} \leq \firstBroadcast{v_{i+1}}{\rho'}$ if and only if $\lastBroadcast{v_i}{\rho} \leq \firstBroadcast{v_{i+1}}{\rho}$.
%	\end{itemize}
	We show that we can build $\rho_K$ by induction on $K$:
	for $K = 1$, there is nothing to do and $\rho_1 = \rho$. Let $1 < K < \ell$, and assume we have built $\rho_{K-1} = C_0 \transup{v^0, t^0} C_1 \transup{v^1, t^1} \cdots \transup{v^{n-1}, t^{n-1}} C_n$ such that $C_n (\Gamma, L_n)$ and:
	\begin{itemize}
		\item for all $v \in \set{v_{K}, \dots, v_\ell}$, $L_n(v) = L(v)$;
		\item for all $1 \leq i \leq K-2$, $\lastBroadcast{v_i}{\rho_{K-1}} \leq \firstBroadcast{v_{i+1}}{\rho_{K-1}}$;
		\item for all $K \leq i \leq \ell$, $\lastBroadcast{v_i}{\rho_{K-1}} \leq \firstBroadcast{v_{i+1}}{\rho_{K-1}}$ if and only if $\lastBroadcast{v_i}{\rho} \leq \firstBroadcast{v_{i+1}}{\rho}$.
	\end{itemize}
	Assume $\lastBroadcast{v_{K-1}}{\rho_{K-1}} > \firstBroadcast{v_K}{\rho_{K-1}}$, then $\lastBroadcast{v_{K-1}}{\rho_{K-1}} \geq 0$ and $v_{K-1}$ issues at least one transition in $\rho_{K-1}$ after $\firstBroadcast{v_{K}}{\rho_{K-1}}$. Denote $j_1 = \min\set{j > \firstBroadcast{v_K}{\rho_{K-1}}\text{ and } C_j \transup{v_{K-1}, t} C_{j+1} \text{ for some } t \in \Delta}$.
	We now build the following sequence of configuration $C'_{j_1}, \dots C'_n$:
	\begin{itemize}
		\item $C'_{j_1} = C'_{j_1 +1 } =C_{j_1}$;
		\item for $j_1 + 1 \leq j < n$, $C'_{j+1} = (\Gamma, L'_{j+1})$ and 
		\begin{itemize}
			\item $L'_{j+1}(v) = L_{j+1}(v)$ for all $v \in \set{v_{K+1}, \dots, v_\ell}$, 
			\item $L'_{j+1}(v) = L_{j+1}(v)$ for all $v \in \set{v_1, \dots, v_{K-2}}$,
			\item $L'_{j+1}(v_{K-1})$ is defined as follows: if $v^j = v_K$ and $t^j $ is a broadcast transition of some message $m \in \Sigma$, and $(L'_j(v_{K-1}) ,?m, p) \in \Delta$ for some $p \in Q$, then $L'_{j+1}(v_{K-1}) = p$, otherwise $L'_{j+1}(v_{K-1}) = L'_j(v_{K-1})$;
			\item $L'_{j+1}(v_{K})$ is defined as follows: 
			\begin{itemize}
				\item if $v^j = v_{K+1}$ and $L'_j(v_K) \neq L_j(v_K)$ and $t^j $ is a broadcast transition of some message $m \in \Sigma$, and $(L'_j(v_{K}), ?m, p) \in \Delta$ for some $p \in Q$, then $L'_{j+1}(v_{K}) = p$;
				\item if $v^j = v_{K+1}$ and $L'_j(v_K) = L_j(v_K)$, then $L'_{j+1}(v_{K}) = L_{j+1}(v_K)$;
				\item if $v^j = v_K$ and $L'_j(v_K) = L_j(v_K)$, then $L'_{j+1}(v_K) = L_{j+1}(v_K)$;
				\item otherwise, $L'_{j+1}(v_K) = L'_j(v_K)$.
			\end{itemize}
		\end{itemize}
	\end{itemize}
	
	Observe that from $C_{j_1}$ to $C_{j_1+1}$ was a transition issued by $v_{K-1}$, after the first broadcast of $v_K$. We have built configurations $C'_{j_1+1}$, \dots $C'_n$ such
	that all actions of $v_{K-1}$ are suppressed, while maintaining an execution. 
	
	Formally, we ow prove that for all $j_1 < j \leq n$,
	\begin{itemize}
	\item $P_1(j)$: either $C'_{j-1} \transup{v^{j-1}, t^{j-1}} C'_{j}$ anf $v^j\in \set{v_K, \dots, v_\ell}$ or $C'_{j} = C'_{j-1}$ and $v^{j-1} \in \set{v_1, \dots v_{K}}$
	\item $P_2(j)$: for all $j_1 + 1 \leq j \leq n$, $L'_j(v_K) = L_j(v_K)$ or $L_j(v_K) \in Q_2^r$. 
	\end{itemize}
	
	Note that when $v^j = v_K$, both $C'_{j-1} \transup{v^{j-1}, t^{j-1}} C'_{j}$  and $C'_{j-1} = C'_j$ are possible, as we will see, this will depends on condition $P_2(j)$.
	
	We prove $P_1(j)$ and $P_2(j)$ by induction on $j$.
	For $j = j_1+1$, $P_1(j)$ trivially holds as $C'_{j_1 +1 }= C'_{j_1}$ and $C_{j_1}\transup{v_{K-1}, t} C_{j_1 +1}$. Let us prove now that $P_2(j)$ holds: recall 
	first that $L'_{j_1 +1}(v_K) = L'_{j_1}(v_K) = L_{j_1}(v_K)$. Since $C_{j_1}\transup{v_{K-1}, t} C_{j_1 +1}$, either $L_{j_1 + 1}(v_K) = L_{j_1}(v_K)$ and $P_2(j)$ holds, or $(L_{j_1}(v_K), ?m, L_{j_1+1}(v_K)) \in \Delta$ and $t=(p,!!m,q)$. 
	Since $j_1 > \firstBroadcast{v_{K}}{\rho_{K-1}}$ and $\PP$ is 2-phase-bounded, $L_{j_1}(v_K) \in Q_1^b\cup Q_2^b \cup Q_2^r$ and so $L_{j_1+1}(v_K) \in Q_2^r$. Hence $P_2(j)$ holds.
	
	Let now $j_1 \leq j < n-1$ such that $P_1(j)$ and $P_2(j)$ hold. 
%	First observe that if $v^j \in \set{v_1, \dots v_{K-1}}$, then $C'_j = C'_{j+1}$.
As a preliminary observe that if $C_1 \transup{v,t} C_1'$ with $C_1 = (\Gamma, L_1)$ and $C'_1 = (\Gamma, L'_1)$ and there exist two configurations $C_2 = (\Gamma, L_2), C_2' = (\Gamma, L'_2)$ are two configurations such that, for all $u \in \set{v}\cup \Neigh{v}$, $L_2(u) = L_1(u)$ and $L_2'(u) = L_1'(u)$, and for all $u\nin \set{v}\cup \Neigh{v}$, $L'_2(u) = L_2(u)$, then $C_2 \transup{v,t} C_2'$.

	Let us now focus on $v^j \in \Vert{\Gamma}$.
	\begin{itemize}
		\item if $v^j \in \set{v_{K+2}, \dots, v_\ell}$ then for all $v \in \set{v^j} \cup \Neigh{v^j}$, by definition, $L'_j(v) = L_j(v)$ and $L'_{i+1}(v) = L_{i+1}(v)$. Furthermore, for all $v \nin \set{v^j} \cup \Neigh{v^j}$, either $v \in \set{v_1, \dots, v_K}$ and $L'_{j+1}(v) = L'_j(v)$, or $v \in \set{v_{K+1}, \dots, v_\ell}$ and $L'_{j+1}(v) = L_{j+1}(v) = L_j(v) = L'_j(v)$. This allows us to conclude that $C'_j \transup{v^j ,t^j} C'_{j+1}$ and so $P_1(j+1)$ holds. Let us show now that $P_2(j+1)$ holds: to this end it suffices to observe that $L'_{j+1}(v_K) = L'_j(v_K)$ and $L_{j+1}(v_K) = L_j(v_K)$ and apply induction hypothesis.
		\item if $v^j =v_{K+1}$ or $v^j = v_K$ and $L'_j(v_K) = L_j(v_K)$, first observe that by construction, $L_{j+1}(v^j) = L'_{j+1}(v^j)$ and $L_j(v^j) = L'_j(v^j)$.
		Observe that $v^j$ has at most two neighbours $v, v'$ such that:
		\begin{itemize}
			\item $v = v_{K+2}$ or $ v =v_{K+1}$, and so by construction $L_{j+1}(v) = L'_{j+1}(v)$ and $L_j(v) = L'_j(v)$;
			\item $v' = v_{K}$ or $v' = v_{K-1}$.
			If $v' = v_{K-1}$ or $v' = v_K$ and $L'_j(v_K) \neq L_j(v_K)$, then by construction either $t^j$ is a broadcast transition of some message $m \in \Sigma$ and $(L'_j(v'), ?m , L'_{j+1}(v')) \in \Delta$. Or, $t^j$ is internal or it is a broadcast transition of a message $m$ and there is no state $p$ such that $(L'_j(v'), ?m , p) \in \Delta$, and $L'_{j+1}(v')) = L'_{j}(v')$.
			
			If $v' = v_K$ and $L'_j(v_K) = L_j(v_K)$, then $L'_{j+1}(v_K) = L_{j+1}(v_K)$ by definition.
			% Furthermore $v^j = v_{K+1}$ and as $C_i \transup{v^j, t} C_{i+1}$, either $(L_j(v_K), ?m, L_{j+1}(v_K)) \in \Delta$ and $t^j$ is a broadcast transition of message $m \in \Sigma$, or $L_j(v_K) = L_{j+1}(v_K)$ and $t^j$ is either internal, or a broadcast of a message $m$ and there is no state $p$ such that $(L_j(v_K), ?m , p) \in \Delta$, and $L'_{j+1}(v')) = L'_{j}(v')$.
		\end{itemize}
		Furthermore, for all $v \nin \set{v^j} \cup \Neigh{v^j}$, either $v \in \set{v_1, \dots, v_K}$ and $L'_{j+1}(v) = L'_j(v)$, or $v \in \set{v_{K+1}, \dots, v_\ell}$ and $L'_{j+1}(v) = L_{j+1}(v) = L_j(v) = L'_j(v)$. This allows us to conclude that $C'_j \transup{v^j ,t^j} C'_{j+1}$ and so $P_1(j+1)$ holds. Let us now show that $P_2(j+1)$ holds: if $v^j = v_K$ and $L'_j(v_K) = L_j(v_K)$, then by construction $L'_{j+1}(v_K) = L_{j+1}(v_K)$ and so $P_2(j+1)$ trivially holds. If $v^j = v_{K-1}$, then either $L'_j(v_K) = L_j(v_K)$ and so by construction, $L'_{j+1}(v_K) = L_{j+1}(v_K)$, or $L'_j(v_K) \neq L_j(v_K)$ and so by induction hypothesis $L_j(v_K) \in Q_2^r$, as $\PP$ is 2-phase-bounded, $L_{j+1}(v_K) \in Q_2^r$.
		
		\item if $v^j = v_K$ and $L'_j(v_K) \neq L_j(v_K)$, then, by induction hypothesis, $L_j(v_K) \in Q_2^r$. Hence, $t$ is an internal transition, and so $L_{j+1}(v_{K+1}) = L_j(v_{K+1}) = L'_j(v_{K+1}) = L'_{j+1}(v_{K+1})$. As a consequence,
		 $C'_{j+1} = C'_j$. Furthermore, by induction hypothesis, $L_j(v_K) \in Q_2^r$ and so, as $\PP$ is 2-phase-bounded, it holds that $L_{j+1}(v_K) \in Q_2^r$.
		 
		 \item if $v^j \in \set{v_1, \dots, v_{K-1}}$, then for all $v \in \set{v_{K+1}, \dots, v_\ell}$, $L_{j+1}(v) = L_j(v)$ and so $C'_{j+1} = C'_j$ and $P_1(j+1)$ holds. Furthermore, either $L_j(v_K) = L_{j+1}(v_K)$ or $(L_j(v_K), ?m, L_{j+1}(v_K))\in \Delta$. In the first case, either $L'_{j+1}(v_K) = L'_{j}(v_K) = L_{j+1}(v_K)$ or $L_j(v_K)= L_{j+1}(v_K) \in Q_2^r$ and so $P_2(j+1)$ holds. In the latter case, as $j > \firstBroadcast{v_K}{\rho_{K-1}}$, by definition of a 2-phase-bounded protocol, $L_j(v_K) \in Q_1^b \cup Q_2^b\cup Q_2^r$ hence, $L_{j+1}(v_K) \in Q_2^r$ and so $P_2(j+1)$ holds.
	\end{itemize}
	
	
	Hence, we have built $C'_{j_1+1} \dots C'_n$ such that $C_0 \trans^\ast C_{j_1} = C'_{j_1 +1}	\trans^\ast C'_n$ and $v_{K-1}$ does not issue any transition between $C'_{j_1 +1}$ and $C'_n$. Furthermore, any node $v \in \set{v_{K+1}, \dots, v_\ell}$ performs the same sequence of transitions and they do so in the same order and $L'_n(v) = L_n(v)$. This concludes the proof.
\end{proof}

By symmetry, we get the following lemma.
\begin{lemma}\label{lemma:CoverLine-2pb-inP:execution-shape-left}
	Let $\rho = C_0\trans^\ast C$ with $C = (\Gamma, L)$ and $1 < K \leq \ell$. 
	There exists $\rho' = C_0  \trans^\ast C'$ such that $C' = (\Gamma, L')$, and 
	\begin{itemize}
		\item for all $v \in \set{v_{1}, \dots, v_{K-1}}$, $L'(v) = L(v)$;
		\item for all $K+1 \leq i \leq \ell$, $\lastBroadcast{v_i}{\rho'} \leq \firstBroadcast{v_{i-1}}{\rho'}$;
		\item for all $1\leq i \leq K-1$, $\lastBroadcast{v_i}{\rho'} \leq \firstBroadcast{v_{i-1}}{\rho'}$ if and only if $\lastBroadcast{v_i}{\rho} \leq \firstBroadcast{v_{i-1}}{\rho}$.
	\end{itemize}
\end{lemma}

We are now ready to prove \cref{lemma:CoverLine-2pb-inP:execution-shape-1}.

\begin{proofof}{\cref{lemma:CoverLine-2pb-inP:execution-shape-1}}
	From $\rho = C_0 \trans^\ast C$ with $C = (\Gamma, L)$ we apply \cref{lemma:CoverLine-2pb-inP:execution-shape-right}\ for $K = N-1$ and we get an execution $\rho' = C'_0 \trans^\ast C'$ such that $C'= (\Gamma, L')$ and 
	\begin{itemize}
		\item for all $v \in \set{v_{N}, \dots, v_\ell}$, $L'(v) = L(v)$;
		\item for all $1 \leq i \leq N-2$, $\lastBroadcast{v_i}{\rho'} \leq \firstBroadcast{v_{i+1}}{\rho'}$;
		\item for all $N\leq i \leq \ell$, $\lastBroadcast{v_i}{\rho'} \leq \firstBroadcast{v_{i+1}}{\rho'}$ if and only if $\lastBroadcast{v_i}{\rho} \leq \firstBroadcast{v_{i+1}}{\rho}$.
	\end{itemize}
	Next, from $\rho'$, we apply \cref{lemma:CoverLine-2pb-inP:execution-shape-left}\ for $K = N+1$ and we get an execution $\rho'' = C''_0 \trans^\ast C''$ such that $C'' = (\Gamma, L'')$ and
	\begin{itemize}
		\item for all $v \in \set{v_{1}, \dots, v_{N}}$, $L''(v) = L'(v)$;
		\item for all $N+2 \leq i \leq \ell$, $\lastBroadcast{v_i}{\rho''} \leq \firstBroadcast{v_{i-1}}{\rho''}$;
		\item for all $1\leq i \leq N$, $\lastBroadcast{v_i}{\rho''} \leq \firstBroadcast{v_{i-1}}{\rho''}$ if and only if $\lastBroadcast{v_i}{\rho'} \leq \firstBroadcast{v_{i-1}}{\rho'}$.
	\end{itemize}
Hence, $\rho''$ covers $q_f$ as $L''(v_N) = L'(v_N) = L(v_N) = q_f$ and 
\begin{itemize}
	\item for all $N+2 \leq i \leq \ell$, $\lastBroadcast{v_i}{\rho''} \leq \firstBroadcast{v_{i-1}}{\rho''}$;
	\item for all $1\leq i \leq N-2$, $\lastBroadcast{v_i}{\rho''} \leq \firstBroadcast{v_{i+1}}{\rho''}$.
\end{itemize}
\end{proofof}


\paragraph{Proof of \cref{lemma:CoverLine-2pb-inP:execution-shape-2}}
We are now ready to prove \cref{lemma:CoverLine-2pb-inP:execution-shape-2}.
We start by three observations which hold independently of if $\PP$ is 2-phase-bounded or not. 
In a line $\Gamma = (V, E)$ with $V = \set{v_1, \dots v_\ell}$ and $E = \set{\langle v_i, v_{i+1} \rangle \mid 1 \leq i < \ell}$, we define the distance between two nodes $v_i, v_j$ as $d(v_i, v_j) = |j-i|$.
\begin{observation}\label{obs:CoverLine-2pb-inP:reordening-broadcasts}
	Let $C, C' \in \CC$, and $u,v \in \Vert{\Gamma}$ such that $d(v,u) \geq 3$, then if $C \transup{u,t} C_1 \transup{v,t'} C'$ for two transitions $t, t' \in \Delta$ and a configuration $C_1 \in \CC$, then there exists $C_2 \in \CC$ such that $C \transup{v,t'} C_2 \transup{u,t} C'$.
\end{observation}

\begin{observation}\label{obs:CoverLine-2pb-inP:reordening-internal-2}
	Let $C, C' \in \CC$, and $u,v \in \Vert{\Gamma}$ such that $d(u, v) \geq 2$. Then if $C \transup{u,t} C_1 \transup{v,t'} C'$ for two transitions $t, t' \in \Delta$ with one of the two transitions \emph{internal} and a configuration $C_1 \in \CC$, then there exists $C_2 \in \CC$ such that $C \transup{v,t'} C_2 \transup{u,t} C'$.
\end{observation}

\begin{observation}\label{obs:CoverLine-2pb-inP:reordening-internal-1}
	Let $C, C' \in \CC$, and $u,v \in \Vert{\Gamma}$. Then if $C \transup{u,t} C_1 \transup{v,t'} C'$ for two internal transitions $t, t' \in \Delta$ and a configuration $C_1 \in \CC$, then there exists $C_2 \in \CC$ such that $C \transup{v,t'} C_2 \transup{u,t} C'$.
\end{observation}

For the rest of this proof we let $\rho = C_0 \transup{v^0, t^0} C_1 \transup{c^1, t^1} \cdots \transup{v^{n-1}, t^{n-1}} C_n$ be the execution obtained from \cref{lemma:CoverLine-2pb-inP:execution-shape-1}. We define $j_1 := \lastBroadcast{v_{N-3}}{\rho} + 1$ and $j_2 = \lastBroadcast{v_{N+3}}{\rho} + 1$.

\begin{lemma}\label{lemma:CoverLine-2pb-inP:delay-1}
	Let $0 \leq j < j_1$ the maximal index such that $C_j \transup{v^j, t^j} C_{j+1}$, for some $v^j \in \set{v_{N-1}, v_N, \dots, v_\ell}$
	then,
	$C_0 \trans^\ast C_j \transup{v^{j+1}, t^{j+1}} C'_{j+1} \trans^\ast C'_{j_1 -2} \transup{v_{N-3}, t^{j_1}} C'_{j_1 - 1} \transup{v^j,t^j} C_{j_1}$.
\end{lemma}
\begin{proof}
	Let $0 \leq j < j_1$ be the maximal index such that $C_j\transup{v^j,t^j} C_{j+1}$ for some $v \in \set{v_{N-1}, v_{N}, \dots v_{\ell}}$.
	
	Recall that $j_1 = \lastBroadcast{v_{N-3}}{\rho} + 1$, and recall that $ \lastBroadcast{v_{N-3}}{\rho} \leq \firstBroadcast{v_{N-2}}{\rho}$, hence either $\firstBroadcast{v_{N-2}}{\rho} = -1$ and so it never broadcast anything, either $j_1 \leq \firstBroadcast{v_{N-2}}{\rho}$.
	In both cases, $v_{N-2}$ does not broadcast anything between $C_0$ and $C_{j_1}$.

	
	As $j$ is maximal, for all $j <k < j_1$, $v^{k} \in \set{v_1, \dots, v_{N-2}}$ and if $v^{k} = v_{N-2}$, $t^{k}$ is internal. 
	We prove by induction that for all $j \leq  k < j_1$: there exists $C'_{j+1} ,\dots ,C'_{k}$ such that $C_{j}\transup{v^{j+1}, t^{j+1}} C'_{j+1} \trans \cdots \transup{v^{k},t^{k}} C'_{k} \transup{v^{j}, t^j} C_{k+1}$. 
	For $k = j$, the induction property triviailly holds. Let $j \leq k <j_1 - 1$ such that $C_{j}\transup{v^{j+1}, t^{j+1}} C'_{j+1} \cdots \transup{v^{k},t^{k}} C'_{k} \transup{v^{j}, t^j} C_{k+1}$. Denote $C_{k+1} \transup{v^{k+1}, t^{k+1}} C_{k+2}$. 
	
	\textbf{First case: $v^j = v_{N-1}$.} Then, note that $\lastBroadcast{v^{k+1}}{\rho} \leq \firstBroadcast{v_{N-1}}{\rho}$, hence $t^j$ is an internal transition as $j < k \leq \lastBroadcast{v^k}{\rho}$. If $v^{k+1} \in \set{v_1, \dots, v_{N-3}}$, then $d(v_{N-1}, v^{k+1}) \geq 2$ and we apply \cref{obs:CoverLine-2pb-inP:reordening-internal-1}, to get that there exists $C'_{k+1}$ such that $C'_{k} \transup{v^{k+1}, t^{k+1}} C'_{k+1} \transup{v^j, t^j} C_{k+2}$. If $v^{k+1} = v_{N-2}$, then $t^{k+1}$ is internal and we can hence apply \cref{obs:CoverLine-2pb-inP:reordening-internal-2}\ to get that there exists $C'_{k+1}$ such that $C'_{k} \transup{v^{k+1}, t^{k+1}} C'_{k+1} \transup{v^j, t^j} C_{k+2}$.
	
	\textbf{Second case: $v^j = v_{N}$.} Then, if $v^{k+1} \in \set{v_1, \dots v_{N-3}}$ and so $d(v_N, v^{k+1}) \geq 3$. We can apply \cref{obs:CoverLine-2pb-inP:reordening-broadcasts}\ to get that there exists $C'_{k+1}$ such that $C'_{k} \transup{v^{k+1}, t^{k+1}} C'_{k+1} \transup{v^j, t^j} C_{k+2}$. Otherwise, $v^{k +1} = v_{N-2}$ and $t^{k+1}$ is internal and $d(v_N, v_{N-2}) = 2$ and so we can apply \cref{obs:CoverLine-2pb-inP:reordening-internal-1}\ to get that there exists $C'_{k+1}$ such that $C'_{k} \transup{v^{k+1}, t^{k+1}} C'_{k+1} \transup{v^j, t^j} C_{k+2}$.
	
	\textbf{Third case: $v^j\in \set{v_{N+1}, \dots v_\ell}$.} Then $d(v^j, v^{k+1}) \geq 3$ and so we can apply \cref{obs:CoverLine-2pb-inP:reordening-broadcasts}\ to get that there exists $C'_{k+1}$ such that $C'_{k} \transup{v^{k+1}, t^{k+1}} C'_{k+1} \transup{v^j, t^j} C_{k+2}$.
	
%	If $v^{j+1} \set{v_1, \dots, v_{N-3}}$, then $d(v^j, v^{j+1}) \geq 3$
\end{proof}

\begin{lemma}\label{lemma:CoverLine-2pb-inP:delay-2}
	Let $j_1 \leq j < j_2$ the \emph{maximal} index such that $C_j \transup{v^j, t^j} C_{j+1}$, for some $v^j \in \set{v_{N-2}, v_{N-1}, v_{N}, v_{N+1}}$, then,
	$C_{j_1} \trans^\ast C_j \transup{v^{j+1}, t^{j+1}} C'_{j+1} \transup{v^{j+2}, t^{j+2}} \cdots \trans C'_{j_2-2} \transup{v_{N+3}, t^{j_2}} C'_{j_2 - 1} \transup{v,t} C_{j_2}$.
\end{lemma}
\begin{proof}
	Let $j_1 \leq j < j_2$ be the maximal index such that $C_j\transup{v^j,t^j} C_{j+1}$ for some $v \in \set{v_{N-2}, v_{N-1}, v_N, v_{N+1}}$.
	
Recall that $j_1 = \lastBroadcast{v_{N-3}}{\rho} +1$, and that $\lastBroadcast{v_{N-3}}{\rho}  \geq \firstBroadcast{v_{N-3}}{\rho} \geq \lastBroadcast{v_{N-2}}{\rho}$, and so by a simple inductive reasoning: $j_1 > \lastBroadcast{v}{\rho}$ for all $v \in \set{v_1, \dots, v_{N-3}}$. Hence, for all $j_1 \leq k  < j_2$, $v^k \nin \set{v_1, \dots, v_{N-3}}$.
	
	Hence, as $j$ is maximal, for all $j <k < j_1$, $v^{k} \in \set{v_{N+2}, \dots, v_{\ell}}$. 
	We prove by induction that for all $j \leq k < j_2$, there exist $C'_{j+1}, \dots C'_k$ such that $C_j\transup{v^{j+1}, t^{j+1}} C'_{j+1} \trans \cdots C'_k \transup{v^j, t^j} C_{k+1}$.
	For $k =j$, the induction property trivially holds. Let $j \leq k <j_2-1$ such that there exist $C'_{j+1}, \dots C'_k$ with $C_j\transup{v^{j+1}, t^{j+1}} C'_{j+1} \trans \cdots C'_k \transup{v^j, t^j} C_{k+1}$. Denote $C_{k+1} \transup{v^{k+1}, t^{k+1}} C_{k+2}$.
	
	\textbf{First case:} $v^j = v_{N+1}$. Then, note that $\lastBroadcast{v^j}{\rho} \leq \firstBroadcast{v_{N+1}}{\rho}$ and so $t^j$ is an internal transition as $j < k+1 \leq \lastBroadcast{v^{k+1}}{\rho}$. If $v^{k+1} \in \set{v_{N+3}, \dots v_\ell}$ then $d(v_{N+1}, v^{k+1}) \geq 2$ and we can apply \cref{obs:CoverLine-2pb-inP:reordening-internal-2}\ to get that there exists $C'_{k+1}$ such that $C'_k \transup{v^{k+1}, t^{k+1}} C'_{k+1}\transup{v^j, t^j}  C_{k+2}$. Otherwise, $v^{k+1} = v_{N+2}$. Recall that $j_2 = \lastBroadcast{v_{N+3}}{\rho} +1$ and that $k+1\leq \lastBroadcast{v_{N+3}}{\rho} \leq \firstBroadcast{v_{N+2}}{\rho}$, hence $t^{k+1}$ is an internal transition. Hence we can apply \cref{obs:CoverLine-2pb-inP:reordening-internal-1}\ to get that there exists $C'_{k+1}$ such that $C'_k \transup{v^{k+1}, t^{k+1}} C'_{k+1}\transup{v^j, t^j}  C_{k+2}$. 
	
	\textbf{Second case:} $v^j = v_N$. Then, if $v^{k+1} \in \set{v_{N+3}, \dots v_{\ell}}$ and so $d(v_N, v^{k+1}) \geq 3$. We can apply \cref{obs:CoverLine-2pb-inP:reordening-broadcasts}\ to get that there exists $C'_{k+1}$ such that $C'_{k} \transup{v^{k+1}, t^{k+1}} C'_{k+1} \transup{v^j, t^j} C_{k+2}$. Otherwise, $v^{k +1} = v_{N+2}$ and $t^{k+1}$ is internal and $d(v_N, v_{N+2}) = 2$ and so we can apply \cref{obs:CoverLine-2pb-inP:reordening-internal-1}\ to get that there exists $C'_{k+1}$ such that $C'_{k} \transup{v^{k+1}, t^{k+1}} C'_{k+1} \transup{v^j, t^j} C_{k+2}$.
	
	\textbf{Third case: $v^j\in \set{v_{N-2}, v_{N-1}}$.} Then $d(v^j, v^{k+1}) \geq 3$ and so we can apply \cref{obs:CoverLine-2pb-inP:reordening-broadcasts}\ to get that there exists $C'_{k+1}$ such that $C'_{k} \transup{v^{k+1}, t^{k+1}} C'_{k+1} \transup{v^j, t^j} C_{k+2}$.
	
\end{proof}

We are now ready to prove \cref{lemma:CoverLine-2pb-inP:execution-shape-2}.

\begin{proofof}{\cref{lemma:CoverLine-2pb-inP:execution-shape-2}}
%	From an execution $\rho = C_0 \trans \cdots \trans C_n$ covering $q_f$ obtained from \cref{lemma:CoverLine-2pb-inP:execution-shape-1}\ we denote $j_1 = \lastBroadcast{v_{N-3}}{\rho} + 1$, and w
	We denote $i_1, \dots i_k$ as the indices $0 \leq i_1 < \cdots < i_k  < j_1$ such that $C_{i_j }\transup{v, t_j} C_{i_j +1}$ for some $v \in \set{v_{N+1}, \dots, v_{\ell}}$ and $t_j \in \Delta$. We denote $\textsf{EarlyBirds}[\rho]$\lug{trouver un meilleur nom} the number of such indices.
	
	We build inductively $\rho_0, \rho_1, \dots \rho_{k}$ such that for all $j$, $\rho_j$ is covering $q_f$ and $\textsf{EarlyBirds}[\rho_{j}] = k-j$, and the order of \ref{lemma:CoverLine-2pb-inP:execution-shape-1}\ is conserved, i.e.  for all $1 \leq i \leq N-2$,
	$\lastBroadcast{v_i}{\rho_{k}} \leq \firstBroadcast{v_{i+1}}{\rho_{k}}$ and for all $N+2 \leq i \leq \ell$, $\lastBroadcast{v_i}{\rho_{k}} \leq \firstBroadcast{v_{i-1}}{\rho_{k}}$.
	
	For $j = 0$, define $\rho_0 = \rho$.
	Let $0 \leq j < k$ and denote $\rho_j = C^j_0 \transup{v^0, t^0} C^j_1 \transup{v^1, t^1} \cdots \transup{v^{n-1} t^{n-1}} C^j_n$ and $j_1^j = \lastBroadcast{v_{N-3}}{\rho_j} + 1$. Denote $i$ the maximal index such that $i <j_1^j$ and $C_{i }\transup{v, t} C_{i +1}$ for some $v \in \set{v_{N+1}, \dots, v_{\ell}}$ and $t \in \Delta$. From \cref{lemma:CoverLine-2pb-inP:delay-1}, $C^{j}_0 \trans^\ast C^j_{i} \transup{v^{i+1}, t^{i+1}} C'_{i +1} \transup{v^{i+2}, t^{i+2}}  \cdots \trans C'_{j_1^j - 1} \transup{v,t} C^j_{j_1^j}$, hence we define $\rho_{j+1} = C^{j}_0 \trans^\ast C^j_{i} \trans C'_{i +1} \trans^\ast \trans C'_{j_1^j - 1} \transup{v,t} C^j_{j_1^j} \trans^\ast C_n$. Hence, $j_1^{j+1} = j_1^j - 1$ and it holds that $\textsf{EarlyBirds}[\rho_{j+1}] = \textsf{EarlyBirds}[\rho_j] - 1 = k-(j+1)$. Furthermore, $\rho_{j+1}$ is covering $q_f$.
	
	Observe that now that it might be that the order between operations of $v^i$ and operations of $v^{i+1}, \dots v^{j_1^j - 1}$ might have changed. If $v^i = v_{N-1}$, then $t^i$ is internal and so $\firstBroadcast{v^i}{\rho_{j}} = \firstBroadcast{v^i}{\rho_j} \geq j_1$, furthermore either $\lastBroadcast{v_{N-2}}{\rho_{j+1}} = \lastBroadcast{v_{N-2}}{\rho_j} = -1$ or $\lastBroadcast{v_{N-2}}{\rho_{j+1}} = \lastBroadcast{v_{N-2}}{\rho_j} \geq j_1$. Otherwise, $v^i \in \set{v_{N}, \dots, v_{\ell}}$. Hence for all $1 \leq i \leq N-2$,
	$\lastBroadcast{v_i}{\rho_{j+1} }\leq \firstBroadcast{v_{i+1}}{\rho_{j+1}}$ and for all $N+2 \leq i \leq \ell$, $\lastBroadcast{v_i}{\rho_{j+1} }\leq \firstBroadcast{v_{i-1}}{\rho_{j+1}}$.
	
	
	Hence, we built $\rho_k$ such that $\rho_k = C^k_0 \trans^\ast C^k_{j_1^k} \trans^\ast C^k_{n}$ and nodes issuing transitions between $C^k_0$ and $C^k_{j_1}$ belong to $\set{v_1, \dots, v_{N-3}, v_{N-2}}$. As $j_1^k = \lastBroadcast{v_{N-3}}{\rho_K} + 1 $, either $j_1^k \leq \firstBroadcast{v_{N-2}}{\rho_K}$ or $v_{N-2}$ never broadcasts anything and so $v_{N-2}$ only issues internal transition in $C^k_0 \trans^\ast C^k_{j_1^k}$.
	
	
	With the same reasoning between $C_{j_1}$ and $C_{j_2}$, and applying this time \cref{lemma:CoverLine-2pb-inP:delay-2}, we finally get an execution $\rho' = C'_0 \trans^\ast C'_{j'_1} \trans^\ast C'_{j'_2} \trans^\ast C'_n $ such that:
	\begin{itemize}
		\item for all $1 \leq i \leq N-2$, $\lastBroadcast{v_i}{\rho'} \leq \firstBroadcast{v_{i+1}}{\rho'}$;
		\item for all $N+2 \leq i \leq \ell$, $\lastBroadcast{v_i}{\rho'} \leq \firstBroadcast{v_{i-1}}{\rho'}$.
		\item nodes issuing transitions between $C'_0$ and $C'_{j'_1}$ belong to $\set{v_1, \dots, v_{N-3}, v_{N-2}}$ and $v_{N-2}$ only performs internal transitions;
		\item nodes issuing transitions between $C'_{j'_1}$ and $C'_{j'_2}$ belong to $\set{v_{N+2}, v_{N+3}, \dots, v_{\ell}}$ and $v_{N+2}$ only performs internal transitions;
%		\item nodes issuing transitions between $C_{j_2}$ and $C_{n}$ belong to $\set{v_{N-2}, v_{N-1} , v_N, v_{N+1}, v_{N+2}}$.
	\end{itemize}
where $j'_1 = \lastBroadcast{v_{N-3}}{\rho'} + 1$ and $j'_2 =\lastBroadcast{v_{N+3}}{\rho'} + 1$.
	Assume a node $v \nin \set{v_{N-2}, v_{N-1} , v_N, v_{N+1}, v_{N+2}}$ issues a transition between $C'_{j'_2}$ and $C'_n$, hence by definition, $\lastBroadcast{v}{\rho'} \geq j'_2$.
	Either $v \in \set{v_1, \dots v_{N-3}}$ and so $\lastBroadcast{v}{\rho'} \leq \lastBroadcast{v_{N-3}}{\rho'} < j'_1 <j'_2$ and we reach a contradiction. Or $v \in \set{v_{N+3}, \dots v_{\ell}}$ and so $\lastBroadcast{v}{\rho'} \leq \lastBroadcast{v_{N+3}}{\rho'} < j'_2$ and we reach a contradiction.
\end{proofof}

\subsubsection{Completeness of the reduction}\label{appendix:subsec:CoverLine-inP:lemma:complete}
This part is dedicated to prove the following lemma.
\begin{lemma}\label{lemma:CoverLine-2pb-inP:complete}
	If $q_f$ is coverable with a line topology, then there exist $q_1, q_2 \in H$ such that $C_{q_1, q_2} \trans^\ast C$ and $C = (\Gamma_5, L)$ with $L(v_3)  = q_f$.
\end{lemma}

If $q_f$ is coverable, then let $\rho = C_0 \trans \cdots \trans C_n$ be the execution obtained from \cref{lemma:CoverLine-2pb-inP:execution-shape-2}. We denote $C_i = (\Gamma, L_i)$ for all $0\leq i \leq n$.

We start by proving that $L_{j_1}(v_{N-2}) \in H$ and $L_{j_2}(v_{N+2}) \in H$.

\begin{lemma}\label{lemma:proof:lemma:CoverLine2pb-complete-case0}
	For all $0 \leq j \leq \firstBroadcast{v_1}{\rho}$, $(L_{j}(v_1), \qinit) \in S$.
\end{lemma}
\begin{proof}
	We prove the lemma by induction on $j$.
	For $j = 0$, $L_0(v_1) = \qinit$ and by construction $(\qinit, \qinit) \in S$.
	Let $0 \leq j < \firstBroadcast{v_1}{\rho}$ such that $(L_{j}(v_1), \qinit) \in S$. 
	Denote $C_j \transup{v^j, t^j} C_{j+1}$. Recall that in $\rho$, as $j < j_1$, it holds that $v^j \in \set{v_1, \dots v_{N-2}}$ (\cref{item:lemma:exec-shape-steps} of \cref{lemma:CoverLine-2pb-inP:execution-shape-2}). Furthermore, as $j < \firstBroadcast{v_1}{\rho}$, then $j < \firstBroadcast{v}{\rho}$ for all $v \in \set{v_1, \dots, v_{N-2}}$ (\cref{item:lemma:exec-shape-order} of \cref{lemma:CoverLine-2pb-inP:execution-shape-2}). Hence, $t^j$ is an internal transition. Either $v^j \neq v_1$ and so $L_{j+1}(v_1) = L_j(v_1)$ and there is nothing to do, or $v^j = v_1$ and so $(L_j(v_1), \tau, L_{j+1}(v_1))\in \Delta$ and so, as $(L_j(v_1), \qinit) \in S$, $(L_{j+1}(v_1), \qinit) \in S$ by definition of $S$.
\end{proof}

We adopt the convention that $L_{-1}(v) = \qinit$ for all $v$.
We prove the following lemma by induction on $k$.
%We define $\firstBroadcast{v_0}{\rho} = -1$.

\begin{lemma}\label{lemma:proof:lemma:CoverLine2pb-complete-case-ind}
	For all $1 < k \leq N-2$, 
	if $L_{\firstBroadcast{v_{k-1}}{\rho}}(v_{k-1}) \in H$, then $L_{j}(v_k)\in H$ for all $\firstBroadcast{v_{k-1}}{\rho} \leq j \leq \firstBroadcast{v_{k}}{\rho}$.
\end{lemma}
\begin{proof}
	Let $1 < k \leq N-2$ such that $L_{\firstBroadcast{v_{k-1}}{\rho}}(v_{k-1}) \in H$, we prove the lemma by induction. 
	For ease of readability, denote $j^{k-1} = \firstBroadcast{v_{k-1}}{\rho}$ and $j^k =  \firstBroadcast{v_{k}}{\rho}$.
	By definition of $H$, there exists $q \in Q$ such that $(L_{j_{k-1}}(v_{k-1}),q)\in S$. 
	%Hence, by definition of $S$, then $(\qinit, L_{j_{k-1}}(v_{k-1}))\in S$.
	

	First let us show that for all $0 \leq j \leq j^{k-1}$, $(L_j(v_k), L_{j^{k-1}}(v_{k-1})) \in S$: for $j = 0$, as $(L_{j^{k-1}}(v_{k-1}),q)\in S$, by definition of $S$, $(\qinit, L_{j^{k-1}}(v_{k-1}))\in S$.
	Let now $0 \leq j < j^{k-1}$ and denote $C_j \transup{v^j, t^j} C_{j+1}$. 
	Recall that in $\rho$, as $j < j^{k-1}$, it holds that $v^j \in \set{v_1, \dots v_{N-2}}$ (\cref{item:lemma:exec-shape-steps} of \cref{lemma:CoverLine-2pb-inP:execution-shape-2}). Furthermore, as $j < j^{k-1}$, then $j < \firstBroadcast{v}{\rho}$ for all $v \in \set{v_{k-1}, \dots, v_{N-2}}$ (\cref{item:lemma:exec-shape-order} of \cref{lemma:CoverLine-2pb-inP:execution-shape-2}). Hence, either $t^j$ is an internal transition, or $v^j \in \set{v_1, \dots v_{k-2}}$. In the latter case, $L_{j+1}(v_k) = L_j(v_k)$.
	Otherwise, either $v^j \neq v_k$ and so $L_{j+1}(v_k) = L_j(v_k)$ and there is nothing to do, or $v^j = v_k$ and so $(L_j(v_k), \tau, L_{j+1}(v_k))\in \Delta$ and so, as $(L_j(v_k), L_{j^{k-1}}(v_{k-1})) \in S$, $(L_{j+1}(v_k), L_{j^{k-1}}(v_{k-1})) \in S$ by definition of $S$.
	
	Hence $(L_{j^{k-1}}(v_k), L_{j^{k-1}}(v_{k-1})) \in S$. We now prove that for all $j^{k-1} \leq j \leq j^k$, $(L_j(v_k), L_j(v_{k+1})) \in S$. As we just proved it for $j = j^{k-1}$, let $j^{k-1} \leq j < j^k$, and denote $C_j \transup{v^j, t^j} C_{j+1}$. Note that from \cref{lemma:CoverLine-2pb-inP:execution-shape-2}, we get that
	(a) $v^j \in \set{v_1, \dots, v_{N-2}}$ as $j < \firstBroadcast{v_k}{\rho} < j_1$; (b) as $j \geq j^{k-1}$, it holds that $j \geq \lastBroadcast{v}{\rho}$ for all $v \in \set{v_1, \dots, v_{k-2}}$, hence $v^j \nin  \set{v_1, \dots, v_{k-2}}$; and (c) if $v^j \in \set{v_{k}, \dots v_{N-2}}$, then $t^j$ is an internal transition as $j \leq \firstBroadcast{v_k}{\rho} \leq \firstBroadcast{v}{\rho}$ for all $v\in \set{v_{k}, \dots v_{N-2}}$.
	
	Overall, we get that either $v^j = v_{k-1}$, or $v^j \in \set{v_{k}, \dots, v_{N-2}}$ and $t^j$ is internal. 
	In the first case, all cases ($t^j$ is an internal transition, $t^j$ is a broadcast transition and the message is received by $v_k$, or $t^j$ is a broadcast transition and the message is not received by $v_k$) are covered by our definition of $S$.
	In the latter case, either $v^j \neq v_k$ and $v_k$ and $v_{k-1}$ remain on the same states, or $v^j =v_k$ and this case is covered by our definition of $S$ ($t^j$ is internal).
	
\end{proof}
Hence, as $L_{\firstBroadcast{v_1}{\rho}}(v_1) \in H$ from \cref{lemma:proof:lemma:CoverLine2pb-complete-case0}, by applying inductively \cref{lemma:proof:lemma:CoverLine2pb-complete-case-ind}, we get that $L_{j}(v_{N-2})\in H$ for all $\firstBroadcast{v_{N-3}}{\rho} \leq j \leq \firstBroadcast{v_{N-2}}{\rho}$. As $j_1 = \firstBroadcast{v_{N-3}}{\rho} + 1$, then $L_{j_1}(v_{N-2})\in H$.

With a similar reasoning, we on $v_{N+2}$ and between $C_{j_1}$ and $C_{j_2}$, we get the following lemma.
\begin{lemma}
	$L_{j_1}(v_{N-2}) \in H$ and $L_{j_2}(v_{N+2}) \in H$.
\end{lemma}

Denote $q_1 =L_{j_1}(v_{N-2})$ and $q_2 = L_{j_2}(v_{N+2}) $.  Denote $C_{j_2} \transup{v^{j_2}, t^{j_2}} C_{j_2+1} \transup{v^{j_2 + 1}, t^{j_2 +1}} \cdots \transup{v^{n-1}, t^{n-1}} C_n$. Recall that from \cref{item:lemma:exec-shape-steps} of \cref{lemma:CoverLine-2pb-inP:execution-shape-2}, $v^{j_2}, \dots v^{n-1} \in \set{v_{N-2}, v_{N-1}, v_N, v_{N+1}, v_{N+2}}$. Denote $C_{q_1, q_2} = (\Gamma_5, L_{q_1, q_2})$, recall that $L_{q_1, q_2}(v_i) = L_{j_2}(v_{N-3 + i})$ for all $1 \leq i \leq 5$.
Hence, $C_{q_1, q_2}= C'_0  \transup{v_2^0, t_2^0} C'_1 \transup{v_2^1, t_2^1} \cdots \transup{v_2^{n-j_2-1}, t_2^{n-j_2-1}} C'_{n-j_2}$ where for all $ 0 \leq j \leq n-j_2$: $C'_j = (\Gamma_5, L'_j)$ and $L'_j(v_i)=  L_{j_2+j}(v_{N-3 + i})$ for all $1 \leq i \leq 5$. And for all $ 0 \leq j < n-j_2$: $t_2^j = t^{j_2 + j}$ and if $v^{j_2 + j} = v_{N-3+i}$ for some $1 \leq i \leq 5$, then $v_2^j = v_i$.
\lug{ici je n'ai pas prouvé formellement, qu'en pensez vous }
Hence, $C_{q_1, q_2} \trans^\ast C'_{n-j_2}$ with $L'_{n-j_2}(v_3) = L_n(v_N) = q_f$.
This concludes the proof of \cref{lemma:CoverLine-2pb-inP:complete}.



\subsubsection{\Iflong{Proof of \cref{lemma:CoverLine-2pb-inP:correct}}Correctness of the Reduction}\label{appendix:subsec:CoverLine-inP:lemma:correct}
\Ifshort{
	This part is devoted to prove the following lemma.
\begin{lemma}\label{lemma:CoverLine-2pb-inP:correct}
	If there exist $q_1, q_2 \in H$, $v \in \Vert{\Gamma_5}$, such that $C_{q_1, q_2} \trans^\ast C$ and $C = (\Gamma_5, L)$ with $L(v) = q_f$, then there exist $\Gamma \in \Lines$, $C_0 \in \II$, $C' = (\Gamma, L')\in \CC$ such that $C_0 \trans^\ast C'$ and $L'(v) = q_f$.
\end{lemma}
}
We start by proving the following lemma.
\begin{lemma}\label{lemma:CoverLine-inP:inH-coverable}
	For all $q \in H$, there exists $k \in \nat$ such that $q$ is coverable with a line topology $\Gamma = (\set{v_1, \dots, v_k}, \set{\langle v_i, v_{i+1}\rangle \mid 1 \leq i <k})$ and vertex $v_1$.
\end{lemma}
\begin{proof}
	We will in fact prove that for all $(q_1, q_2) \in S$, there exists $\Gamma_{q_1, q_2} \in \Lines$ such that $\Vert{\Gamma_{q_1, q_2}} = \set{v_1, \dots, v_k}$, $\Edges{\Gamma_{q_1,q_2}} = \set{\langle v_i, v_{i+1} \rangle \mid 1 \leq i <k}$ for some $k \in \nat$ with $k \geq 2$ and there exists $C_0  \in \II$, $C = (\Gamma_{q_1, q_2}, L)$ with $C_0 \trans^\ast C$ and $L(v_1) = q_1$ and $L(v_2) = q_2$.
	
	Denote $S_0, \dots, S_K$ the subsets defined by the algorithm to build $S$. We have $S = S_{N}$.
	We prove the property to be true for all $(q_1, q_2) \in S_i$ by induction on $0 \leq i \leq N$.
	For  $i = 0$, $S_0 = \set{(\qinit, \qinit)}$, this is trivial: define $\Gamma_{\qinit, \qinit} = (\set{v_1,v_2}, \set{\langle v_1, v_2\rangle})$ and take the initial configuration $C = (\Gamma_{\qinit, \qinit}, L_0)$ with $L_0(v_1)=L_0(v_2) = \qinit$.
	Let $0\leq i <K$, and assume we proved the property to be true for all $(q_1,q_2) \in S_i$. 
	Let $(q_1,q_2) \in S_{i+1} \in S_i$.
	\begin{itemize}
		\item if there exists $(q_1, p_2) \in S_i$ such that $(p_2, \tau, q_2) \in \Delta$, let $\Gamma_{q_1, p_2}$, $C_0$ and $C = (\Gamma_{q_1, p_2}, L)$ obtained from the induction hypothesis such that $C_0 \trans^\ast C$ and $L(v_1) = q_1$ and $L(v_2) = p_2$. Then, $C \transup{v_2, (p_2, \tau, q_2)} C'$ and $C' = (\Gamma_{q_1, p_2}, L')$ with $L'(v_1) = q_1$ and $L'(v_2) = q_2$;
		
		\item if there exists $(p_1, q_2) \in S_i$ such that $(p_1, \tau, q_1) \in \Delta$, the reasoning is the same as in the previous case;
		
		\item if there exists $(p_1, p_2) \in S_i$ and $m \in \Sigma$ such that $(p_1, ?m, q_1) \in \Delta$ and $(p_2, !!m, q_2) \in \Delta$, we use a similar reasoning as in the previous cases;
		%then let $\Gamma_{p_1, p_2}$, $C_0$ and $C = (\Gamma_{p_1, p_2}, L)$ obtained from the induction hypothesis such that $C_0 \trans^\ast C$ and $L(v_1) = p_1$ and $L(v_2) = p_2$. Then, $C \transup{v_2, (p_2, !!m, q_2)} C'$ and $C' = (\Gamma_{p_1, p_2}, L')$ with $L'(v_1) = q_1$ and $L'(v_2) = q_2$;
		
		\item  if there exists $(q_1, p_2) \in S_i$ and $m \in \Sigma$ such that$(p_2, !!m, q_2) \in \Delta$ and $m\nin R(q_1)$, we use a similar reasoning as in the previous cases;
		%then let $\Gamma_{q_1, p_2}$, $C_0$ and $C = (\Gamma_{q_1, p_2}, L)$ obtained from the induction hypothesis such that $C_0 \trans^\ast C$ and $L(v_1) = q_1$ and $L(v_2) = p_2$. Then, $C \transup{v_2, (p_2, !!m, q_2)} C'$ and $C' = (\Gamma_{q_1, p_2}, L')$ with $L'(v_1) = q_1$ and $L'(v_2) = q_2$;
		
		\item if there exists $q_3$ such that $(q_2, q_3) \in S_i$ and $q_1 = \qinit$, then let $\Gamma_{q_2, q_3}$, $C_0$ and $C = (\Gamma_{q_2, q_3}, L)$ obtained from the induction hypothesis such that $C_0 \trans^\ast C$ and $L(v_1) = q_2$ and $L(v_2) = q_3$. Define $\Gamma_{q_1, q_2} = (\set{v'_1} \cup \Vert{\Gamma_{q_2,q_3}}, \set{ \langle v, v_1 \rangle } \cup \Edges{\Gamma_{q_2,q_3}})$. Note that $q_2 \in H \subseteq Q_0 \cup Q_1^r$\lug{not proved formally}, hence between $C_0$ and $C$, $v_1$ does not broadcast anything. 
		Hence, define $C'_0 = (\Gamma_{q_1, q_2}, L_0)$ and $C' = (\Gamma_{q_1, q_2}, L')$ such that for all $v \in \Vert{\Gamma_{q_1, q_2}}$, $L_0(v)= \qinit$ and $L'(v'_1) = \qinit$, and for all $v \in \Vert{\Gamma_{q_2, q_3}}$, 
		$L'(v) = L(v)$.
		Then $C'_0 \trans^\ast C'$, as nodes in $\Vert{\Gamma_{q_2, q_3}}$ can execute the same sequence of steps and $v_1$ does not broadcast anything, hence $v'_1$ stays in $\qinit$. \lug{c'est moins formel que d'habitude car je ne pense pas que ce soit compliqué et on est deja à 45 pages, est ce que ça vous va ? }
	\end{itemize}
	
\end{proof}

\begin{proofof}{\cref{lemma:CoverLine-2pb-inP:correct}}
	Let $q_1, q_2 \in H$, from \cref{lemma:CoverLine-inP:inH-coverable}, let $\Gamma_{q_1} = (\set{v_1, \dots, v_k}, \set{\langle v_i, v_{i+1} \rangle \mid 1 \leq i < k})$, and $\Gamma_{q_2}= (\set{v'_1, \dots, v'_n}, \set{\langle v'_i, v'_{i+1} \rangle \mid 1 \leq i < n})$ the two line topologies such that $q_1$ is coverable with $v_1$ and $q_2$ with $v'_1$.
	Denote $C_0 \trans^\ast C$ with $C = (\Gamma_{q_1}, L)$ and $L(v_1)= q_1$ and $C'_0 \trans^\ast C'$ with $C' = (\Gamma_{q_2}, L')$ and $L'(v'_1)= q_2$. As $q_1, q_2 \in H$ and $H \subseteq Q_0 \cup Q_1^r$, $v_1$ does not broadcast anything between $C_0$ and $C$ and $v'_1$ does not broadcast anything between $C'_0$ and $C'$.
	
	Define $\Gamma = (V, E)$ such that $V = \Vert{\Gamma_{q_1}} \cup \Vert{\Gamma_{q_2}} \cup \set{u_2, u_3,u_4}$ and $E = \Edges{\Gamma_{q_1}}\cup \Edges{\Gamma_{q_2}} \cup \set{\langle v_1, u_2\rangle, \langle u_2, u_3 \rangle, \langle u_3, u_4 \rangle, \langle u_4, v'_1 \rangle}$.
	Note that $v_1$ and $v'_1$ are not neighbours, and that each node in $\Vert{\Gamma_{q_1}}$ [resp. in $\Vert{\Gamma_{q_2}}$] has the same neighbourhood as before.
	Denote $C''_0 = (\Gamma, L''_0)$ with $L''_0(v) = \qinit$ for all $v \in \Vert{\Gamma}$. 
	
	Denote $C_0 \transup{v^1, t^1} C_1 \transup{v^2, t^2} \cdots \transup{v^{n_1}, t^{n_1}} C_{n_1} = C$ and $C'_0 \transup{v'^1, t'^1} C'_1 \transup{v'^2, t'^2} \cdots \transup{v'^{n_2}, t'^{n_2}} C'_{n_2} =  C'$.
	Then $C''_0\transup{v^1, t^1} C''_1 \transup{v^2, t^2} \cdots \transup{v^{n_1}, t^{n_1}} C''_{n_1}\transup{v'^1, t'^1} C''_{n_1 +1} \transup{v'^2, t'^2} \cdots \transup{v'^{n_2}, t'^{n_2}} C''_{n_1 + n_2}$ with $C''_{n_1 + n_2} = (\Gamma, L''_{n_1 + n_2})$ and $L''_{n_1 + n_2}(v) = L_{n_1}(v)$ for all $v \in \Vert{\Gamma_{q_1}}$ and $L''_{n_1 + n_2}(v) = L'_{n_2}(v)$ for all $v \in \Vert{\Gamma_{q_2}}$ and $L''_{n_1 + n_2}(v) = \qinit$ for all $v \in \set{u_2, u_3, u_4}$.
	Hence $L''_{n_1 + n_2}(v_1) = q_1$ and $L''_{n_1 +n_2}(v'_1) = q_2$.
	
	Finally, rename $\Gamma_5 = (\set{u_1, u_2, u_3, u_4, u_5}, \set{\langle u_i, u_{i+1} \rangle \mid 1 \leq i < 5})$, and $v_1$ by $u_1$ and $v'_1$ by $u_5$.
	Denote $C^5_{q_1, q_2} \transup{u^1, \delta^1} C^5_1 \transup{u^2, \delta^2} \cdots \transup{u^{n_3}, t^{n_3}} C^5_{n_3}$. Denote $C^5_{q_1, q_2} = (\Gamma_5, L_{q_1, q_2})$ and $C^5_{n_3} = (\Gamma_5, L^5_{n_3})$ 
	Note that for all $u \in \Vert{\Gamma_5}$, $L_{q_1, q_2}(u) = L''_{n_1 +n_2}(u)$. Hence, $C''_{n_1 + n_2}\transup{u^1, \delta^1} C''_{n_1 +n_2 +1} \transup{u^2, \delta^2} \cdots \transup{u^{n_3}, \delta^{n_2}} C''_{n_1 + n_2 + n_3}$ with $C''_{n_1 + n_2 +n_3} = (\Gamma, L''_{n_1 + n_2 +n_3})$ and $L''_{n_1 + n_2+n_3}(v) = L_{n_1}(v)$ for all $v \in \set{u_1, u_2, u_3, u_4, u_5}$.
	Hence $L''_{n_1 + n_2+n_3}(u_3) = q_f$.
	\lug{c'est moins formel que d'habitude car je ne pense pas que ce soit compliqué et on est deja à 45 pages, est ce que ça vous va ? }
	
%	\lugtext{j'en suis là}
	
	
	
\end{proofof}

==> wait-only-section.tex <==
\section{About wait-only protocols}



\begin{theorem}
	\Cover\ and \CoverTree\ are in P for wait-only protocols
\end{theorem}
\color{violet} proof uses copycat property\color{black}

\begin{theorem}
	\CoverLine\ is undecidable for wait-only protocols
\end{theorem}
\color{violet} proof reduction inspired from reduction of the general case\color{black}

